Pathways on the Image Manifold: Image Editing via Video Generation

Recent advances in image editing, driven by image diffusion models, have shown remarkable progress. However, significant challenges remain, as these models often struggle to follow complex edit instructions accurately and frequently compromise fidelity by altering key elements of the original image. Simultaneously, video generation has made remarkable strides, with models that effectively function as consistent and continuous world simulators. In this paper, we propose merging these two fields by utilizing image-to-video models for image editing. We reformulate image editing as a temporal process, using pretrained video models to create smooth transitions from the original image to the desired edit. This approach traverses the image manifold continuously, ensuring consistent edits while preserving the original image's key aspects. Our approach achieves state-of-the-art results on text-based image editing, demonstrating significant improvements in both edit accuracy and image preservation. Visit our project page at https://rotsteinnoam.github.io/Frame2Frame.

==> outline.tex <==


introduction changes:
1. add our strengths:
    - actions
    - lighting
    - more tasks?
2. add world simulators (sora paper), natural interpolations
3. unlike editing tasks that don't have a lot of data, video generators enjoy endless data
4. here or future work- should improve more in the future as these models improve.

